3D-Aware Object Goal Navigation via Simultaneous Exploration and Identification

Object goal navigation (ObjectNav) in unseen environments is a fundamental task for Embodied AI. Agents in existing works learn ObjectNav policies based on 2D maps, scene graphs, or image sequences. Considering this task happens in 3D space, a 3D-aware agent can advance its ObjectNav capability via learning from fine-grained spatial information. However, leveraging 3D scene representation can be prohibitively unpractical for policy learning in this floor-level task, due to low sample efficiency and expensive computational cost. In this work, we propose a framework for the challenging 3D-aware ObjectNav based on two straightforward sub-policies. The two sub-polices, namely corner-guided exploration policy and category-aware identification policy, simultaneously perform by utilizing online fused 3D points as observation. Through extensive experiments, we show that this framework can dramatically improve the performance in ObjectNav through learning from 3D scene representation. Our framework achieves the best performance among all modular-based methods on the Matterport3D and Gibson datasets, while requiring (up to 30x) less computational cost for training.

==> fig/consistency.tex <==
\begin{wrapfigure}{r}{7cm}
% \centering
% \vspace{-0.5cm}

\begin{overpic}
% []
%[width=\linewidth,grid,tics=10]
[width=0.5\textwidth]
{fig/img/semantic_consistency.pdf}
    % \put(12,30.5){\footnotesize (a)}
    % \put(38,30.5){\footnotesize (b)}
    % \put(65,30.5){\footnotesize (c)}
    % \put(87.5,30.5){\footnotesize (d)}
\end{overpic}
\caption{
Illustration of octree update. The connections and semantic predictions of per-point octree will be online updated.
}
\vspace{-0.2cm}
\label{fig:consistency}
\end{wrapfigure}


==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> table/ablation.tex <==
\begin{table}[!t]\centering
% \vspace{-5pt}
\scalebox{1}{
\setlength{\tabcolsep}{1.0}{
\begin{tabular}{cccc|ccc}
\hline
\multirow{2}{*}{2D map} & \multicolumn{2}{c}{3D points} & \multirow{2}{*}{V. Policy} & \multirow{2}{*}{SPL(\%)} & \multirow{2}{*}{Succ.(\%)} & \multirow{2}{*}{DTS(m)} \\
& Pos. & KL div. & &\\
\hline
    \checkmark &            &            & 
        &  13.1  &  31.4  &  4.971  \\
               & \checkmark & \checkmark & 
        &  12.9  &  30.8  &  4.931 \\
    \checkmark & \checkmark &            & 
        &  10.2  &  10.2  &  35.4 \\
    \checkmark & \checkmark & \checkmark & 
        &  10.2  &  10.2  &  35.4 \\
    \checkmark & \checkmark & \checkmark & \checkmark
        &  14.6  &  -  &  4.74 \\ 
\hline

\end{tabular}
}}
\caption{Ablation Study}
\label{tab:ablation}
\end{table} 

==> table/mp3d.tex <==
\begin{table}[!t]\centering
\caption{
ObjectNav validation results on MP3D. Baselines are adapted from \cite{ramakrishnan2022poni}, \cite{chaplot2020object}. Note that, the SemExp and Stubborn do not report the results on MP3D validation. We therefore faithfully provide the results, denoted with *, by evaluating the pre-trainedmo model from their open available code. 
}
% \vspace{-5pt}
\scalebox{1}{
\setlength{\tabcolsep}{1}{
\begin{tabular}{l|ccc}
\hline
Method      & SPL(\%)\uparrow       & Succ.(\%)\uparrow    & DTS(m)\downarrow         \\ \hline \hline
DD-PPO      & 1.8           & 8.0           & 6.9           \\
Red-Rabbit  & 7.9           & 34.6          & -             \\
THDA        & 11.0          & 28.4          & 5.6           \\
Habitat-Web & 10.2          & 35.4 & -             \\ 
\hline
FBE         & 7.2           & 22.7          & 6.7           \\
ANS         & 9.2           & 27.3          & 5.8           \\
L2M         & 13.3          & 34.3          & 3.49          \\
Stubborn*    & 13.5          & 31.2          & 5.02          \\
SemExp*      & 10.9          & 28.3          & 6.06          \\
PONI        & 12.1          & 31.8          & 5.10          \\
Ours        & 14.8          & 34.2          & 4.64 \\ \hline
\end{tabular}
}}
\label{tab:main_results}
\end{table} 

==> table/mp3d_gibson.tex <==
\begin{table}[!t]\centering
\caption{
ObjectNav validation results on MP3D and Gibson. Baselines are adapted from \cite{ramakrishnan2022poni}, \cite{chaplot2020object}. Note that, the SemExp and Stubborn do not report the results on MP3D validation. We therefore faithfully provide the results, denoted with *, by evaluating the pre-trainedmo model from their open available code. 
}
% \vspace{-5pt}
\scalebox{1}{
\setlength{\tabcolsep}{1.0}{
\begin{tabular}{l|ccc|ccc}
\hline
            & \multicolumn{3}{c|}{Gibson (val)}             & \multicolumn{3}{c}{Mappterport 3D (val)}      \\ \cline{2-7} 
Method      & SPL(\%)\uparrow       & Succ.(\%)\uparrow     & DTS(m)\downarrow        & SPL(\%)\uparrow       & Succ.(\%)\uparrow     & DTS(m)\downarrow        \\ \hline \hline
DD-PPO      & 10.7          & 15.0          & 3.24          & 1.8           & 8.0           & 6.9           \\
Red-Rabbit  & -             & -             & -             & 7.9           & 34.6          & -             \\
THAD        & -             & -             & -             & 11.1          & 28.4          & 5.58          \\
Habitat-Web & -             & -             & -             & 10.2          & \textbf{35.4} & -             \\ \hline
FBE         & 28.3          & 64.3          & 1.78          & 7.2           & 22.7          & 6.7           \\
ANS         & 34.9          & 67.1          & 1.66          & 9.2           & 27.3          & 5.8           \\
L2M         & -             & -             & -             & 11.0          & 32.1          & 5.12          \\
SemExp*      & 39.6          & 71.7          & 1.39          & 10.9          & 28.3          & 6.06          \\
Stubborn*    & -             & -             & -             & 13.5          & 31.2          & 5.01          \\
PONI        & 41.0          & \textbf{73.6} & 1.25          & 12.1          & 31.8          & 5.10          \\
Ours        & \textbf{41.7} & 72.5          & \textbf{1.21} & \textbf{14.6} & 34.0          & \textbf{4.74} \\ \hline
\end{tabular}
}}
\label{tab:main_results}
\end{table} 

==> table/mp3d_gibson_all_name.tex <==
\begin{table}[!t]\centering
\caption{
ObjectNav validation results on MP3D and Gibson. Baselines are adapted from \cite{ramakrishnan2022poni}, \cite{chaplot2020object}. Note that, the L2M, SemExp and Stubborn do not report the results on MP3D validation. We therefore faithfully provide the results, denoted with *, by evaluating the pre-trainedmo model from their open available code. 
}
% \vspace{-5pt}
\scalebox{0.95}{
\setlength{\tabcolsep}{0.95}{
\begin{tabular}{l|ccc|ccc}
\hline
            & \multicolumn{3}{c|}{Gibson (val)}             & \multicolumn{3}{c}{Mappterport 3D (val)}      \\ \cline{2-7} 
Method      & SPL(\%)\uparrow       & Succ.(\%)\uparrow     & DTS(m)\downarrow        & SPL(\%)\uparrow       & Succ.(\%)\uparrow     & DTS(m)\downarrow        \\ \hline \hline
DD-PPO~\cite{wijmans2019dd}     & 10.7          & 15.0          & 3.24          & 1.8           & 8.0           & 6.90           \\
Red-Rabbit~\cite{ye2021auxiliary}  & -             & -             & -             & 7.9           & 34.6          & -             \\
THAD~\cite{maksymets2021thda}      & -             & -             & -             & 11.1          & 28.4          & 5.58          \\
Habitat-Web~\cite{ramrakhya2022habitat} & -             & -             & -             & 10.2          & \textbf{35.4} & -             \\ \hline
FBE~\cite{Robotics1997Proceedings1I}        & 28.3          & 64.3          & 1.78          & 7.2           & 22.7          & 6.70           \\
ANS~\cite{chaplot2020learning}         & 34.9          & 67.1          & 1.66          & 9.2           & 27.3          & 5.80           \\
L2M~\cite{georgakis2022l2m}         & -             & -             & -             & 11.0          & 32.1          & 5.12          \\
SemExp*~\cite{chaplot2020object}      & 39.6          & 71.7          & 1.39          & 10.9          & 28.3          & 6.06          \\
Stubborn*~\cite{luo2022stubborn}    & -             & -             & -             & 13.5          & 31.2          & 5.01          \\
PONI~\cite{ramakrishnan2022poni}        & 41.0          & \textbf{73.6} & 1.25          & 12.1          & 31.8          & 5.10          \\
\hline
Ours        & \textbf{41.7} & 72.5          & \textbf{1.21} & \textbf{14.8} & 32.6          & \textbf{4.04} \\ \hline
\end{tabular}
}}
\label{tab:main_results}
\end{table} 

==> table/row_table.tex <==
\begin{minipage}[t]{0.48\textwidth}
\centering
\makeatletter\def\@captype{table}
\caption{Comparison of verification policy.}
\scalebox{0.85}{
\setlength{\tabcolsep}{0.85}{
\begin{tabular}{l|cc|ccc}
\hline
\multirow{2}{*}{Method}        & \multicolumn{2}{c|}{Type} & \multicolumn{1}{l}{\multirow{2}{*}{SPL(\%)}} & \multicolumn{1}{l}{\multirow{2}{*}{Succ.(\%)}} & \multicolumn{1}{l}{\multirow{2}{*}{DTS(m)}} \\
& Repr.  & Thre. \\ 
\hline \hline
\multirow{4}{*}{Deterministic} 
    &  2D  &  0.75  &  13.0  &  29.7  &  5.168  \\
    &  2D  &  0.85  &  12.8  &  30.1  &  5.151  \\
    &  3D  &  0.75  &  13.7  &  32.3  &  4.179  \\ 
    &  3D  &  0.85  &  13.5  &  31.5  &  4.386  \\ 
\hline
Learning (Ours)
    & 3D   &  -     &  \textbf{14.8}  &  \textbf{32.6}  &  \textbf{4.036}  \\ 
\hline
\end{tabular}}}
\label{tab:verification}
\end{minipage}
\begin{minipage}[t]{0.48\textwidth}
\makeatletter\def\@captype{table}
\caption{Ablation study of proposed method.}
\scalebox{0.85}{
\setlength{\tabcolsep}{0.85}{
\begin{tabular}{cccc|ccc}
\hline
\multirow{2}{*}{2D map} & \multicolumn{2}{c}{3D points} & \multirow{2}{*}{V. Policy} & \multirow{2}{*}{SPL(\%)} & \multirow{2}{*}{Succ.(\%)} & \multirow{2}{*}{DTS(m)} \\
& Pos. & KL div. & &\\
\hline \hline
    \checkmark &            &            & 
        &  13.1  &  31.4  &  4.971   \\
               & \checkmark & \checkmark & 
        &  12.9  &  30.8  &  4.931  \\
    \checkmark & \checkmark &            & 
        &  13.5  &  32.4  &  4.810  \\
    \checkmark & \checkmark & \checkmark & 
        &  13.7  &  32.3  &  4.179  \\
\hline
    \checkmark & \checkmark & \checkmark & \checkmark
        &  \textbf{14.8}  &  \textbf{32.6}  &  \textbf{4.036}  \\ 
\hline
\end{tabular}}}
\label{tab:ablation}
\end{minipage}
\end{minipage}


==> table/study_explore.tex <==
\begin{wraptable}{r}{7cm}
\vspace{-8pt}
\scalebox{1}{
\setlength{\tabcolsep}{1.0}{
\begin{tabular}{l|cccc}
\hline
Method & SPL(\%) & S.SPL(\%) & Succ.(\%) & DTS(m) \\
\hline \hline
    L. C. 
        &  11.2  &  19.5  &  29.2  &  5.063  \\
    L. Grid D.
        &  13.0  &  20.9  &  31.5  &  4.944  \\
    L. 8 D.
        &  13.6  &  21.6  &  31.7  &  4.692  \\
    H. 4 D. 
        &  14.4  &  22.9  &  32.1  &  5.024  \\
\hline
    L. 4 D. (Ours)
        &  13.7  &  22.1  &  32.3  &  4.179  \\ 
\hline
\end{tabular}
}}
\caption{Comparison of exploration policy. L. indicates Learning based, C. indicates continuous global goal, D. indicates discrete direction. }
\label{tab:exploration}
\end{wraptable} 

==> table/study_stop.tex <==
\begin{table}
% \vspace{-5pt}
\scalebox{1}{
\setlength{\tabcolsep}{1.0}{
\caption{Comparison of stopping strategies}
\begin{tabular}{l|cc|ccc}
\hline
\multirow{2}{*}{Method}        & \multicolumn{2}{c|}{Type} & \multicolumn{1}{l}{\multirow{2}{*}{SPL(\%)}} & \multicolumn{1}{l}{\multirow{2}{*}{Succ.(\%)}} & \multicolumn{1}{l}{\multirow{2}{*}{DTS(m)}} \\
& Repr.  & Thre. \\ 
\hline \hline
\multirow{4}{*}{Deterministic} 
    &  2D  &  0.75  &  13.0  &  29.7  &  5.168  \\
    &  2D  &  0.85  &  12.8  &  30.1  &  5.151  \\
    &  3D  &  0.75  &  13.7  &  32.3  &  4.179  \\ 
    &  3D  &  0.85  &  13.5  &  31.5  &  4.386  \\ 
\hline
Learning (Ours)
    & 3D   &  -     &  14.8  &  32.6  &  4.036  \\ 
\hline
\end{tabular}}}
\label{tab:exploration}
\end{table} 

==> table/study_stop1.tex <==
\begin{table}[!t]\centering
% \vspace{-5pt}
\scalebox{1}{
\setlength{\tabcolsep}{1}{
\begin{tabular}{l|cc|cccc}
\hline
\multirow{2}{*}{Method}        & \multicolumn{2}{c|}{Type} & \multicolumn{1}{l}{\multirow{2}{*}{SPL(\%)}} & \multicolumn{1}{l}{\multirow{2}{*}{S.SPL(\%)}} & \multicolumn{1}{l}{\multirow{2}{*}{Succ.(\%)}} & \multicolumn{1}{l}{\multirow{2}{*}{DTS(m)}} \\
                               & Repr.  & Thre. & \multicolumn{1}{l}{}                         & \multicolumn{1}{l}{}                             & \multicolumn{1}{l}{}                           & \multicolumn{1}{l}{}                        \\ \hline \hline
\multirow{4}{*}{Deterministic} & 2D            & 0.75      & 13.0                                         & 21.4                                             & 29.7                                           & 5.158                                       \\
                               & 2D            & 0.85      & 12.8                                         & 21.0                                             & 30.1                                           & 5.151                                       \\
                               & 3D            & 0.75      & -                                            & -                                                & -                                              & -                                           \\
                               & 3D            & 0.85      & -                                            & -                                                & -                                              &                                             \\ \hline
Learning (Ours)                       & 3D            & -         & -                                            & -                                                & -                                              & -                                           \\ \hline
\end{tabular}
}}
\caption{
Study on Stop Policy. 
}
\label{tab:verification}
\end{table} 

==> table/sup_heuristic.tex <==
\begin{table}[!h] \centering
\begin{tabular}{l|cccc}
\hline
Method & SPL(\%) & SoftSPL(\%) & Succ.(\%) & DTS(m) \\
\hline
Our w/o HGS
    &  13.7  &  22.7  &  31.1  &  5.189  \\
Our
    &  \textbf{14.8}  &  \textbf{23.2}  &  \textbf{32.6}  &  \textbf{4.036}  \\
\hline

\end{tabular}
\caption{Results on L2M Dataset.}
\label{tab:sup_heu}
\end{table} 

==> table/tab_mp3d_l2m.tex <==
\begin{table}[!t]\centering
\caption{
ObjectNav validation results on MP3D and Gibson. Baselines are adapted from \cite{ramakrishnan2022poni}, \cite{chaplot2020object}. Note that, the L2M, SemExp and Stubborn do not report the results on MP3D validation. We therefore faithfully provide the results, denoted with *, by evaluating the pre-trainedmo model from their open available code. 
}
% \vspace{-5pt}
\scalebox{1.0}{
\setlength{\tabcolsep}{1.0}{
\begin{tabular}{lcccc}
\hline
\multicolumn{1}{c}{}                                      & \multicolumn{4}{c}{Mappterport 3D (val)}                                                         \\ \hline
\multicolumn{1}{l|}{Method}                               & SPL(\%)\uparrow & \multicolumn{1}{l}{SoftSPL(\%)\uparrow} & Succ.(\%)\uparrow & DTS(m)\downarrow \\ \hline
\multicolumn{1}{l|}{FBE~\cite{Robotics1997Proceedings1I}} & 7.2             & 7.2                                     & 22.7              & 6.70             \\
\multicolumn{1}{l|}{ANS~\cite{chaplot2020learning}}       & 9.2             & 9.2                                     & 27.3              & 5.80             \\
\multicolumn{1}{l|}{L2M~\cite{georgakis2022l2m}}          & 11.0            & 11.0                                    & 32.1              & 5.12             \\
\multicolumn{1}{l|}{SemExp*~\cite{chaplot2020object}}     & 10.9            & 10.9                                    & 28.3              & 6.06             \\
\multicolumn{1}{l|}{Stubborn*~\cite{luo2022stubborn}}     & 13.5            & 13.5                                    & 31.2              & 5.01             \\
\multicolumn{1}{l|}{PONI~\cite{ramakrishnan2022poni}}     & 12.1            & 12.1                                    & 31.8              & 5.10             \\ \hline
\multicolumn{1}{l|}{Ours}                                 & \textbf{14.8}   & \textbf{14.8}                           & 32.6              & \textbf{4.04}    \\ \hline
\multicolumn{1}{c}{}                                      & \multicolumn{4}{c}{L2M Dataset (L2M split)}                                                      \\ \hline
\multicolumn{1}{l|}{Method}                               & SPL(\%)\uparrow & \multicolumn{1}{l}{SoftSPL(\%)\uparrow} & Succ.(\%)\uparrow & DTS(m)\downarrow \\ \hline
\multicolumn{1}{l|}{SemExp*~\cite{chaplot2020object}}     & 10.9            & 10.9                                    & 28.3              & 6.06             \\
\multicolumn{1}{l|}{Stubborn*~\cite{luo2022stubborn}}     & 13.5            & 13.5                                    & 31.2              & 5.01             \\
\multicolumn{1}{l|}{Ours}                                 & \textbf{14.8}   & \textbf{14.8}                           & 32.6              & \textbf{4.04}    \\ \hline
\end{tabular}
}}
\vspace{-0.2cm}
\label{tab:mp3d}
\end{table} 
